BASE Layers: Simplifying Training of Large, Sparse Models

We introduce a new balanced assignment of experts (BASE) layer for large language models that greatly simplifies existing high capacity sparse layers. Sparse layers can dramatically improve the efficiency of training and inference by routing each token to specialized expert modules that contain only a small fraction of the model parameters. However, it can be difficult to learn balanced routing functions that make full use of the available experts; existing approaches typically use routing heuristics or auxiliary expert-balancing loss functions. In contrast, we formulate token-to-expert allocation as a linear assignment problem, allowing an optimal assignment in which each expert receives an equal number of tokens. This optimal assignment scheme improves efficiency by guaranteeing balanced compute loads, and also simplifies training by not requiring any new hyperparameters or auxiliary losses. Code is publicly released at https://github.com/pytorch/fairseq/

==> plots/gshard_top.tex <==
\addplot coordinates {(0.052,56.55) (0.105,23.97) (0.157,16.91) (0.210,14.81) (0.262,13.64) (0.314,12.98) (0.369,12.43) (0.422,12) (0.475,11.69) (0.528,11.36) (0.581,11.14) (0.635,10.95) (0.688,10.78) (0.742,10.6) (0.795,10.44) (0.849,10.31) (0.904,10.19) (0.959,10.07) (1.013,9.97) (1.067,9.86)};

==> plots/moe_2layer.tex <==

\addplot coordinates {(0.051,38.05) (0.100,30.35) (0.148,16.58) (0.197,14.12) (0.246,12.99) (0.295,12.22) (0.343,11.63) (0.392,11.18) (0.440,10.85) (0.489,10.54) (0.538,10.34) (0.587,10.15) (0.636,9.96) (0.685,9.8) (0.734,9.62) (0.784,9.52) (0.832,9.4) (0.881,9.28) (0.930,9.17) (0.980,9.05) (1.029,8.95) (1.078,8.87) (1.127,8.78) (1.176,8.7) (1.225,8.62) (1.274,8.55) (1.323,8.45) (1.372,8.42) (1.421,8.33) (1.470,8.25) (1.519,8.19) (1.568,8.13) (1.617,8.09) (1.666,8.04) (1.715,7.99) (1.764,7.94) (1.813,7.88) (1.862,7.81) (1.911,7.75) (1.960,7.7) (2.009,7.63)};

==> plots/moe_interleave.tex <==
% jan15_intermediate/stdout/lm_route_interleave.model_lr0.0005_freq8_distance_dotproduct_centroid_lr_1.0_delta0_sandwich0.0_routing_auction_layers24_10_warmup2000_ffratio0.72_dim2048_heads16_gpu128_seq1024.34888464
\addplot coordinates {(0.003,11102.1) (0.004,5949.62) (0.082,62.82) (0.164,27.31) (0.245,20.05) (0.328,16.65) (0.410,15.11) (0.490,14.22) (0.569,13.6) (0.647,13.14) (0.724,12.75) (0.803,12.43) (0.881,12.21) (0.959,11.96) (1.037,11.74) (1.115,11.58) (1.194,11.4) (1.273,11.26) (1.351,11.1) (1.431,10.98) (1.512,10.84) (1.593,10.73) (1.672,10.62) (1.752,10.51) (1.834,10.42) (1.916,10.32) (1.999,10.24) (2.082,10.14) (2.164,10.07) (2.246,9.99) (2.329,9.93) (2.412,9.88) (2.494,9.86) (2.515,9.86)};

==> plots/moe_no_shuffle.tex <==
\addplot coordinates {(0.046,53.09) (0.092,23.76) (0.138,17.17) (0.183,14.95) (0.228,13.79) (0.273,12.97) (0.318,12.44) (0.363,12.01) (0.408,11.61) (0.453,11.37) (0.498,11.11) (0.543,10.88) (0.588,10.7) (0.633,10.51) (0.678,10.35) (0.724,10.22) (0.769,10.1) (0.815,9.97) (0.860,9.84) (0.906,9.73) (0.951,9.62) (0.996,9.53) (1.041,9.45) (1.087,9.38) (1.132,9.29) (1.177,9.21) (1.222,9.11) (1.267,9.05) (1.312,9) (1.357,8.93) (1.401,8.89) (1.447,8.81) (1.492,8.76) (1.537,8.7) (1.582,8.64) (1.627,8.59) (1.673,8.52) (1.719,8.48) (1.764,8.41) (1.810,8.35) (1.855,8.3) (1.901,8.27) (1.946,8.22) (1.992,8.18) (2.038,8.14) (2.084,8.11) (2.129,8.04) (2.175,8.01) (2.220,7.98) (2.266,7.94) (2.280,7.92) (2.311,7.89) (2.357,7.87) (2.402,7.85) (2.447,7.83) (2.492,7.82) (2.537,7.82) (2.548,7.82)};

==> plots/switch_top.tex <==
\addplot coordinates {(0.043,65.28) (0.087,26.35) (0.130,18.09) (0.173,15.63) (0.215,14.37) (0.258,13.58) (0.300,13.03) (0.344,12.64) (0.389,12.3) (0.433,12) (0.477,11.78) (0.522,11.61) (0.567,11.46) (0.611,11.25) (0.655,11.14)};
